BiLO-CPDP: Bi-Level Programming for Automated Model Discovery in Cross-Project Defect Prediction

Cross-Project Defect Prediction (CPDP), which borrows data from similar projects by combining a transfer learner with a classifier, have emerged as a promising way to predict software defects when the available data about the target project is insufficient. How-ever, developing such a model is challenge because it is difficult to determine the right combination of transfer learner and classifier along with their optimal hyper-parameter settings. In this paper, we propose a tool, dubbedBiLO-CPDP, which is the first of its kind to formulate the automated CPDP model discovery from the perspective of bi-level programming. In particular, the bi-level programming proceeds the optimization with two nested levels in a hierarchical manner. Specifically, the upper-level optimization routine is designed to search for the right combination of transfer learner and classifier while the nested lower-level optimization routine aims to optimize the corresponding hyper-parameter settings.To evaluateBiLO-CPDP, we conduct experiments on 20 projects to compare it with a total of 21 existing CPDP techniques, along with its single-level optimization variant and Auto-Sklearn, a state-of-the-art automated machine learning tool. Empirical results show that BiLO-CPDP champions better prediction performance than all other 21 existing CPDP techniques on 70% of the projects, while be-ing overwhelmingly superior to Auto-Sklearn and its single-level optimization variant on all cases. Furthermore, the unique bi-level formalization inBiLO-CPDP also permits to allocate more budget to the upper-level, which significantly boosts the performance.

==> tables/c_old.tex <==
\begin{table*}[htbp]
	\centering
	\caption{Overview of 16 selected classifiers ([N], [R] and [C] denote integer, real and categorical value, respectively).}
	\label{tab:classifier}%
	\vspace{-0.5em}
	\scalebox{0.5}{
	\addtolength{\tabcolsep}{-3pt}
	\begin{tabular}{c|p{9.11em}|p{18.665em}|p{9.835em}||rrrr}
	\hline
	\multicolumn{1}{c|}{\multirow{1}[4]{*}{\textbf{Classification techniques }}} & \multicolumn{3}{p{30.055em}<{\centering}||}{ \textbf{Parameters }}  & \multicolumn{1}{c|}{\multirow{1}[4]{*}{\textbf{Classification techniques }}} & \multicolumn{3}{p{30.055em}<{\centering}}{\textbf{Parameters }} \\
	\cline{2-4}\cline{6-8}          & \centering \textbf{Name } & \centering \textbf{Description } & \centering \textbf{Range } & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}<{\centering}|}{\textbf{Name }} & \multicolumn{1}{p{21.555em}<{\centering}|}{\textbf{Description }} & \multicolumn{1}{p{9.11em}<{\centering}}{\textbf{Range }} \\
	\hline
	\multicolumn{1}{c|}{\multirow{3}[4]{*}{\texttt{K-Nearest Neighbor (KNN)}}} & n\_eighbors & The number of neighbors to each point (default=1) [N] & [1, 50] & \multicolumn{1}{c|}{\multirow{8}[10]{*}{\texttt{Support Vector Machine (SVM)}}} & \multicolumn{1}{p{8.5em}|}{C} & \multicolumn{1}{p{21.555em}|}{Regularization parameter (default=1) [R]} & \multicolumn{1}{p{9.11em}}{[0.001, 10]} \\
	\cline{2-4}\cline{6-8}          & p     & The power parameter for the Minkowski metric (default=2) [N] & [1, 5] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{kernel} & \multicolumn{1}{p{21.555em}|}{The type of kernel (default= poly) [C]} & \multicolumn{1}{p{9.11em}}{{ rbf,  linear,  poly,  sigmoid}} \\
	\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{8}[10]{*}{\texttt{Decision Tree (DT)}}} & max\_eatures & The maximum number of estimators (default=10) [N] & [10, 100] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{degree} & \multicolumn{1}{p{21.555em}|}{Degree of the polynomial kernel function (default=3) [N]} & \multicolumn{1}{p{9.11em}}{[1, 5]} \\
	\cline{2-4}\cline{6-8}          & criterion & The function to measure the quality of a split (default= gini) [C] & { gini,  entropy} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{coef0} & \multicolumn{1}{p{21.555em}|}{Independent term in kernel function. It is only significant in  poly nd  sigmoid default=0.0) [R]} & \multicolumn{1}{p{9.11em}}{[0, 10]} \\
	\cline{2-4}\cline{6-8}          & min\_samples\_leaf & \textcolor[rgb]{ .129,  .145,  .161}{The minimum number of samples required to be at a leaf node (default=1) [N]} & [1, 20] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{gamma} & \multicolumn{1}{p{21.555em}|}{Kernel coefficient for  rbf,  poly nd  sigmoid default=1) [R]} & \multicolumn{1}{p{9.11em}}{[0.01, 100]} \\
	\cline{2-8}          & splitter & The number of features to consider when looking for the best split (default= auto) [C] & { auto,  sqrt,  log2} & \multicolumn{1}{c|}{\multirow{4}[8]{*}{\texttt{Multi-layer Perceptron (MLP)}}} & \multicolumn{1}{p{8.5em}|}{active} & \multicolumn{1}{p{21.555em}|}{Activation function for the hidden layer (default= relu) [C]} & \multicolumn{1}{p{9.11em}}{{ identity,  logistic,  tanh,  relu}} \\
	\cline{2-4}\cline{6-8}          & min\_amples\_plit & The minimum number of samples required to split an internal node (default=2) [N] & [2, N\_ource/10] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{hidden\_layer\_size} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{The number of neurons in the i-th hidden layer (default=100) [N]}} & \multicolumn{1}{p{9.11em}}{[50, 200]} \\
	\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{5}[10]{*}{\texttt{Random Forest (RF)}}} & n\_stimators & The maximum number of estimators (default=10) [N] & [10, 100] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{solver} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{The solver for weight optimization (default=adam) [C]}} & \multicolumn{1}{p{9.11em}}{{lbfgs, sgd, adam}} \\
	\cline{2-4}\cline{6-8}          & criterion & The function to measure the quality of a split (default= gini) [C] & { gini,  entropy} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{iter} & \multicolumn{1}{p{21.555em}|}{Maximum number of iterations (default=200) [N]} & \multicolumn{1}{p{9.11em}}{[100, 250]} \\
	\cline{2-8}          & max\_eatures & The number of features to consider when looking for the best split (default= auto) [C] & { auto,  sqrt,  log2} & \multicolumn{1}{c|}{\multirow{3}[6]{*}{\texttt{Ridge}}} & \multicolumn{1}{p{8.5em}|}{alpha} & \multicolumn{1}{p{21.555em}|}{Regularization strength (default=1) [R]} & \multicolumn{1}{p{9.11em}}{[0.0001, 1000]} \\
	\cline{2-4}\cline{6-8}          & min\_samples\_leaf & \textcolor[rgb]{ .129,  .145,  .161}{The minimum number of samples required to be at a leaf node (default=1) [N]} & [1, 20] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{fit\_intercept} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{Whether to calculate the intercept for this model (default=False) [C]}} & \multicolumn{1}{p{9.11em}}{{ True,  False}} \\
	\cline{2-4}\cline{6-8}          & min\_samples\_plit & The minimum number of samples required to split an internal node (default=2) [N] & [2, N\_ource/10] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{tol} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{Precision of the solution (default=0.001) [R]}} & \multicolumn{1}{p{9.11em}}{[0.00001, 0.1]} \\
	\hline
	\multicolumn{1}{c|}{\multirow{3}[6]{*}{\texttt{Logistic Regression (LR)}}} & penalty & \textcolor[rgb]{ .129,  .145,  .161}{Used to specify the norm used in the penalization (default=L2) [C]} & {L1, L2} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\texttt{Radius Neighbors Classifier (RNC)}}} & \multicolumn{1}{p{8.5em}|}{radius} & \multicolumn{1}{p{21.555em}|}{Range of parameter space to use by default for radius\_neighbors queries (default=1) [R]} & \multicolumn{1}{p{9.11em}}{[0, 10000]} \\
	\cline{2-4}\cline{6-8}          & fit\_intercept & \textcolor[rgb]{ .129,  .145,  .161}{Whether to calculate the intercept for this model (default=False) [C]} & { True,  False} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{weight} & \multicolumn{1}{p{21.555em}|}{Weight function used in prediction (default=uniform) [C]} & \multicolumn{1}{p{9.11em}}{{uniform, distance}} \\
	\cline{2-8}          & tol   & \textcolor[rgb]{ .129,  .145,  .161}{Precision of the solution (default=0.001) [R]} & [0.00001, 0.1] & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textcolor[rgb]{ .129,  .145,  .161}{\texttt{Nearest centroid classifier (NCC)}}}} & \multicolumn{1}{p{8.5em}|}{metric} & \multicolumn{1}{p{21.555em}|}{The metric of distance (default=enclidean) [C]} & \multicolumn{1}{p{9.11em}}{{euclidean, manhattan, chebyshev, minkowski, mahalanobis}} \\
	\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{4}[8]{*}{\texttt{Perceptron}}} & penalty & \textcolor[rgb]{ .129,  .145,  .161}{Used to specify the norm used in the penalization (default=L2) [C]} & {L1, L2} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{\textcolor[rgb]{ .129,  .145,  .161}{shrink\_threshold}} & \multicolumn{1}{p{21.555em}|}{Threshold for shrinking centroids to remove features (default=0) [R]} & \multicolumn{1}{p{9.11em}}{[0, 10]} \\
	\cline{2-8}          & alpha & Constant that multiplies the regularization term (default=0.0001) [R] & [0.00001,0.1] & \multicolumn{1}{c|}{\multirow{5}[10]{*}{\texttt{Extra Tree Classifier (EXtree)}}} & \multicolumn{1}{p{8.5em}|}{max\_eatures} & \multicolumn{1}{p{21.555em}|}{The maximum number of estimators (default=10) [N]} & \multicolumn{1}{p{9.11em}}{[10, 100]} \\
	\cline{2-4}\cline{6-8}          & fit\_intercept & \textcolor[rgb]{ .129,  .145,  .161}{Whether to calculate the intercept for this model (default=False) [C]} & { True,  False} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{criterion} & \multicolumn{1}{p{21.555em}|}{The function to measure the quality of a split (default= gini) [C]} & \multicolumn{1}{p{9.11em}}{{ gini,  entropy}} \\
	\cline{2-4}\cline{6-8}          & tol   & \textcolor[rgb]{ .129,  .145,  .161}{Precision of the solution (default=0.001) [R]} & [0.00001, 0.1] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{min\_samples\_leaf} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{The minimum number of samples required to be at a leaf node (default=1) [N]}} & \multicolumn{1}{p{9.11em}}{[1, 20]} \\
	\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{5}[10]{*}{\texttt{Extra Trees Classifier (EXs)}}} & max\_eatures & The maximum number of estimators (default=10) [N] & [10, 100] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{splitter} & \multicolumn{1}{p{21.555em}|}{The number of features to consider when looking for the best split (default= random) [C]} & \multicolumn{1}{p{9.11em}}{{ random, best}} \\
	\cline{2-4}\cline{6-8}          & criterion & The function to measure the quality of a split (default= gini) [C] & { gini,  entropy} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{min\_amples\_plit} & \multicolumn{1}{p{21.555em}|}{The minimum number of samples required to split an internal node (default=2) [N]} & \multicolumn{1}{p{9.11em}}{[2, N\_ource/10]} \\
	\cline{2-8}          & min\_samples\_leaf & \textcolor[rgb]{ .129,  .145,  .161}{The minimum number of samples required to be at a leaf node (default=1) [N]} & [1, 20] & \multicolumn{1}{c|}{\multirow{3}[6]{*}{\texttt{Bagging}}} & \multicolumn{1}{p{8.5em}|}{n\_estimators} & \multicolumn{1}{p{21.555em}|}{The number of base estimators in the ensemble (default=100) [N]} & \multicolumn{1}{p{9.11em}}{[10, 200]} \\
	\cline{2-4}\cline{6-8}          & splitter & The number of features to consider when looking for the best split (default= random) [C] & { random, best} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{max\_samples} & \multicolumn{1}{p{21.555em}|}{The number of samples to draw from X to train each base estimator (default=1.0) [R]} & \multicolumn{1}{p{9.11em}}{[0.7, 1.0]} \\
	\cline{2-4}\cline{6-8}          & min\_amples\_plit & The minimum number of samples required to split an internal node (default=2) [N] & [2, N\_ource/10] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{max\_features} & \multicolumn{1}{p{21.555em}|}{The number of features to draw from X to train each base estimator (default=1.0) [R]} & \multicolumn{1}{p{9.11em}}{[0.7, 1.0]} \\
	\hline
	\multicolumn{1}{c|}{\multirow{3}[6]{*}{\texttt{Naive Bayes (NB)}}} & NBType & The type of prior distribution (default= Gaussian) [C] & { gaussian,  multinomial,  complement } & \multicolumn{1}{c|}{\multirow{4}[8]{*}{\textcolor[rgb]{ .129,  .145,  .161}{\texttt{Passive Aggressive Classifier (PAC)}}}} & \multicolumn{1}{p{8.5em}|}{C} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{Maximum step size (regularization) (default=1.0) [R]}} & \multicolumn{1}{p{9.11em}}{[0.001, 100]} \\
	\cline{2-4}\cline{6-8}          & alpha & Additive (Laplace/Lidstone) smoothing parameter for multinomial and complement(default=1.0) [R] & [0, 10] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{fit\_intercept} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{Whether to calculate the intercept for this model (default=False) [C]}} & \multicolumn{1}{p{9.11em}}{{ True,  False}} \\
	\cline{2-4}\cline{6-8}          & norm  & Whether or not a second normalization of the weights is performed (default=False) [C] & { True,  False} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{tol} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{Precision of the solution (default=0.001) [R]}} & \multicolumn{1}{p{9.11em}}{[0.00001, 0.1]} \\
	\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\texttt{adaBoost}}} & n\_estimators & The maximum number of estimators (default=50) [N] & [10, 1000] & \multicolumn{1}{c|}{} & \multicolumn{1}{p{8.5em}|}{loss} & \multicolumn{1}{p{21.555em}|}{\textcolor[rgb]{ .129,  .145,  .161}{The loss function to be used (default=hinge) [C]}} & \multicolumn{1}{p{9.11em}}{{hinge, squared\_hinge}} \\
	\cline{2-8}          & learning\_rate & A factor that shrinks the contribution of each classifier (default=1) [R] & [0.01, 10] &       &       &       &  \\
	\cline{1-4}    \end{tabular}
	}
	\vspace{-1em}
\end{table*}

==> tables/tl_old.tex <==



\begin{table*}[htbp]
    \centering
    \caption{Overview of 13 selected transfer learners ([N], [R] and [C] denote integer, real and categorical value, respectively).}
    \label{tab:transfer_learner}
    \vspace{-0.5em}
	\scalebox{0.63}{
	\addtolength{\tabcolsep}{-2pt}
	\begin{tabular}{c|p{5.89em}<{\centering}|p{19.945em}<{\centering}|p{7.945em}<{\centering}||p{7.8em}<{\centering}|p{5.89em}<{\centering}|p{19.72em}<{\centering}|p{7.72em}<{\centering}}
		\hline
		\multicolumn{1}{c|}{\multirow{1}[4]{*}{\textbf{Algorithms}}} & \multicolumn{3}{m{33.78em}<{\centering}||}{\textbf{Parameters }} & \multirow{1}[4]{*}{\textbf{Algorithms}} & \multicolumn{3}{m{33.05em}<{\centering}}{\textbf{Parameters }} \\
		\cline{2-4}\cline{6-8}          & \textbf{Name } & \textbf{Description } & \textbf{Range} & \multicolumn{1}{c|}{} & \textbf{Name } & \textbf{Description } & \textbf{Range } \\
		\hline
		\multicolumn{1}{c|}{\multirow{4}[4]{*}{\texttt{NNfilter ~\cite{TurhanMBS09} }}} & k     & The number of neighbors to each point (default=10) [N] & $[1,100]$ & \multirow{4}[4]{*}{\texttt{CDE\_SMOTE ~\cite{limsettho2018cross}}} & k     & The number of neighbors to each point (default=10) [N] & $[1,100]$ \\
		\cline{2-4}\cline{6-8}          & metric & The metric of distance (default=Euclidean) [C] & Euclidean, Manhattan, Chebyshev, Minkowski, Mahalanobis & \multicolumn{1}{c|}{} & metric & The metric of distance (default=Euclidean) [C] & Euclidean, Manhattan, Chebyshev, Minkowski, Mahalanobis \\
		\hline
		\multicolumn{1}{c|}{\multirow{5}[6]{*}{\texttt{FSS\_bagging ~\cite{he2013learning}}}} & topN  & The number of closest training sets (default=5) [N] & $[1,15]$ & \multirow{6}[8]{*}{\texttt{CLIFE\_MORPH ~\cite{peters2013balancing}}} & n     & The number of neighbors to each point (default=10) [N] & $[1,100]$ \\
		\cline{2-4}\cline{6-8}          & threshold & The threshold for bagging (default=0.5) [R] & [0.3, 0.7] & \multicolumn{1}{c|}{} & alpha & The lower bound for generated random numbers (default=0.15) [R] & $[0.05,0.2]$ \\
		\cline{2-4}\cline{6-8}          & ratio & The ratio of unstable features filtered out (default=0.2) [R] & $[0.1,0.5]$ & \multicolumn{1}{c|}{} & beta  & The upper bound for generated random numbers (default=0.35) [R] & $[0.2,0.4]$ \\
		\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{5}[8]{*}{\texttt{TCA+ ~\cite{NamPK13}}}} & kernel & The type of kernel (default= linear) [C] & primal,  linear,  rbf,  sam & \multicolumn{1}{c|}{} & percentage & The percentage to remove original data (default=0.8) [R] & $[0.6,0.9]$ \\
		\cline{2-8}          & dimension & The dimension after transfer (default=5) [N] & [5, max(N\_ource, N\_arget)] & \multirow{2}[4]{*}{\texttt{FeSCH ~\cite{ni2017cluster}}} & nt    & The specified number of selected features (default=1) [N] & [1, N\_source] \\
		\cline{2-4}\cline{6-8}          & lamb  & Lambda value in equation (default=1) [R] & $[0.000001,100]$ & \multicolumn{1}{c|}{} & strategy & The feature ranking strategy (default=SFD) [C] & SFD, LDF, FCR \\
		\cline{2-8}          & gamma & Kernel bandwidth for  RBF kernel (default=1) [R] & $[0.00001,100]$ & \texttt{HISNN ~\cite{ryu2015hybrid}} & minham & The radius of a search ring Hamming space (default=1) [N] & [1, N\_source] \\
		\hline
		\multicolumn{1}{c|}{\multirow{3}[4]{*}{\texttt{UM ~\cite{zhang2014towards}}}} & $p$-value & The associated $p$-value for statistical test (default=0.05) [R] & [0.01, 0.1] & \multirow{5}[6]{*}{\texttt{MCWs ~\cite{qiu2018multiple}}} & k     & The number of components (default=2) [N] & [2, N\_group] \\
		\cline{2-4}\cline{6-8}          & quantifyType & The type of quantifying the difference between distributions (default= cliff) [C] & cliff,  cohen & \multicolumn{1}{c|}{} & sigma & The parameter of KMM (default=1) [R] & $[0.01,10]$ \\
		\cline{1-4}\cline{6-8}    \multicolumn{1}{c|}{\multirow{8}[12]{*}{\texttt{GIS ~\cite{hosseini2018benchmark}}}} & prob  & The probability of mutation (default=0.05) [R] & $[0.02,0.1]$ & \multicolumn{1}{c|}{} & lambda & The parameter to control the regularisation term (default=1) [R] & $[0.000001,100]$ \\
		\cline{2-8}          & chrm\_size & The size of each chromosome (default=0.02) [R] & $[0.02,0.1]$ & \multirow{3}[4]{*}{\texttt{TD ~\cite{herbold2013training}}} & strategy & The strategy of selecting source projects (default=NN) [C] & NN, EM \\
		\cline{2-4}\cline{6-8}          & pop\_size & The size of population (default=30) [N] & $[2,30]$ & \multicolumn{1}{c|}{} & k     & The number of desired training sets for NN strategy (default=10) [N] & [1, N\_group] \\
		\cline{2-8}          & num\_parts & The amount of test data divided (default=5) [N] & $[2,6]$ & \multirow{3}[4]{*}{\texttt{VCB ~\cite{ryu2016value}}} & m     &  The maximum number of iterations (default=30) [N] & $[2,30]$ \\
		\cline{2-4}\cline{6-8}          & num\_gens & The number of generations of each genetic optimization run (default=20) [N] & $[5,20]$ & \multicolumn{1}{c|}{} & lambda &  The penalty magnitude (default=1.0) [R] & $[0.5,1.5]$ \\
		\cline{2-8}          & mcount & The number of instances to mutate (default=5) [N] & $[3,10]$ & \texttt{PCAmining ~\cite{nagappan2006mining}} & dimension & The dimension after transfer (default=5) [N] & [5, max(N\_ource, N\_arget)] \\
		\hline
	\end{tabular}
	}
	\vspace{-1em}
\end{table*}

